Concentration of Submodular Functions and Read-k Families Under Negative Dependence

We study the question of whether submodular functions of random variables satisfying various notions of negative dependence satisfy Chernoff-like concentration inequalities. We prove such a concentration inequality for the lower tail when the random variables satisfy negative association or negative regression, partially resolving an open problem raised in (Qiu and Singla [QS22]). Previous work showed such concentration results for random variables that come from specific dependent-rounding algorithms (Chekuri, Vondrak, and Zenklusen [CVZ10] and Harvey and Olver [HO14]). We discuss some applications of our results to combinatorial optimization and beyond. We also show applications to the concentration of read-k families [Gav+15] under certain forms of negative dependence; we further show a simplified proof of the entropy-method approach of [Gav+15].

==> 04_peres-singh-vishnoi.tex <==
\section{Concentration for \cite{innovations/PeresSV17} Rounding Algorithm}

\cite{innovations/PeresSV17} introduce an algorithm for rounding an interior point of a matroid polytope to one of its vertices via a sticky Brownian motion, and show that the resulting random variables satisfy negative association. To implement this in polynomial time, they discretize the process to a Gaussian random walk, and the resulting algorithm gives random variables with an approximate negative association guarantee. We will show that the random variables from their polynomial-time algorithm still have the Chernoff-like concentration properties shown in the previous sections, up to constant factors. This shows that \cite{innovations/PeresSV17} gives the same concentration properties of both randomized pipage rounding and swap rounding, while giving the stronger negative dependence guarantee of approximate negative association.

[give pseudocode for the algorithm, and summarize its main properties. In particular, mention that the fractional $y_t$ satisfies negative association exactly.]


We formalize the intuition, and give the full proof below.

\begin{theorem}
    Fix $\epsilon>0$.
    Let $f$ be a non-negative monotone submodular function with marginal values in $[0,1]$ and let $F$ be the multilinear extension of $f$. Let $(x_1,\ldots,x_n)\in P(\mathcal{M})$ be a point in a matroid polytope, and let $X_1,\ldots,X_n$ be the random vector obtained from it by running Algorithm \textcolor{red}{[PSV17]} with parameter $\epsilon'=\epsilon/n^{2.5}$. If we let, $\mu_0=F(x_1,\ldots,x_n)$ and $\delta>0$, then we have the following:
    $$\Pr[f(X_1,\ldots,X_n)\le (1-\delta)\cdot \mu_0]\le (1+\epsilon)\cdot \exp(-\mu_0\delta^2/2).$$
\end{theorem}

Our proof will proceed in two steps, mirroring the proof of Theorem \ref{thm:main-concentration}. The first part will show that an approximate version of Lemma \ref{lem:exp-mom} still holds for these random variables satisfying approximate negative association. Then we will follow the proof of Theorem \ref{thm:main-concentration} to conclude the Chernoff-type bound.

==> 05_MO_max.tex <==
\section{Multi-objective Maximization of Monotone
Submodular Functions with Cardinality Constraint -- improvement of \cite{udwani2021multiobjective}}
\rv{cited arxiv bcs the journal version has mistakes and different a subroutine for stage 1}
In this section we demonstrate how our concentration result applies for solving multi-objective submodular maximization problem subject to a cardinality constraint in the setting of \cite{udwani2021multiobjective}. Namely, we can improve and simplify the analysis of their algorithm which consists of stages. We replace the independent rounding stage by Srinivasan's dependent rounding procedure\cite{Srinivasan2001DistributionsOL}.

\subsection{Preliminaries and General Overview}
Given a matroid $\mathcal{M}(N,\mathcal{I})$ on a ground set $N$ of cardinality $n$, and given $m$
submodular monotone non-decreasing functions 
$f_1,\ldots,f_m$ on $\mathcal{I}$,
our objective is to find a Pareto set $S\in\mc I$ -- a set that is not dominated by any other $S'\in\mc I$.
In other words, for any $S'\in \mc I$ there exists $1\le i\le m$ such that $f_i(S)>f_i(S')$.
The task to determine whether a set belongs to a collection of Pareto sets is NP-hard, thus, a problem of Pareto set approximation is reasonable to consider instead.
\begin{definition}
    $S$ is an 
\textit{$\varepsilon$-approximate Pareto set} if for any other feasible solution $S'$ there exists $1\le i\le m$ such that $f_i(S')<(1+\veps)f_i(S)$.
\end{definition}
However, we will solve a different problem: 
\label{problem}Given an $m$ real values 
$V_1, . . . , V_m$, we present an algorithm that either returns a solution $S$ with 
$f_i(S)\geq V_i$ for all $i$, or returns a certificate of infeasibility that there is no solution 
$S'$ with 
$f_i(S')\ge V_i(1 + \epsilon)$. For constant $m$, to be able to find this algorithm with running time polynomial in $n$ and $1/\veps$ is equivalent to being able to construct an $\veps-$Pareto set in polynomial time.\cite[Theorem~2]{892068}\\

Throughout this section we consider $\mc M$ to be a $k-$uniform matroid, i.e., any set $S\in I$ is of cardinality $k$. \cite{udwani2021multiobjective} is largely based on Chekuri et al.'s work\cite{focs/ChekuriVZ10} who consider this problem on a general matroid and prove that
there exists an algorithm to find a $(1-1/e-\epsilon)$- approximate Pareto set with the running time polynomial in $n$ (again, using the result from \cite{892068}). Note that that the approach used in the proves only provides a result for an algorithm with running time polynomial in $n$ and $1/\veps$, but exponential in $m$. In contrast, Udwani's results hold for a super constant $m = o(\frac{k}{\log^3 k})$., which is achieved by simplifying the pre-processing step [nah, put this as an observation in the stage itself]

The main result of this section is the following theorem:
\begin{theorem}\label{thm: multi-obj}
    For a $k-$uniform matroid $\mc M = (N, \mc I)$ there exists an algorithm with the running time polynomial in $n$ and $m$ that for any vector $(V_1,\cdots, V_m)\in \mathbb{R}^m_+$ either returns a solution $S\in I$ such that $f_i(S)\ge (1-\veps)(1-1/e)(1-m/k\veps^3)V_i$ for all $i$ with constant probability, or returns a certificate that there is no set $S\in \mc I$ such that $f_i(S)\ge V_i$ holds for every $i$.
\end{theorem}
Note that this is an optimized version of \cite[~Thm 7]{udwani2021multiobjective}. In comparison, the original result contains an additional factor in $(1-\veps)(1-1/e)(1-m/k\veps^3)V_i$ and, hence, has a slower rate of convergence to $(1-1/e)$ as $k\to \infty$.\\

Let us describe the algorithm for solving \ref{problem}. It consists of three stages:\\

\textbf{Stage 1 (Pre-processing):} Choose a subset $S_1$ of the elements with large marginal values, so that for the remaining elements $N-S_1$ their marginal values $f_i(\cdot|S_1)$ are at most $\epsilon^3 V_i$ for any $i$. In the cardinality constraint problem this stage can be done simply using a greedy algorithm for choosing elements in $S_1$. $S_1$ would have at most $1/\epsilon^3$ elements [result].\\

\begin{algorithm}
\caption{Choosing the initial set} \label{pr}
\textbf{Input: }$f_1,\cdots,f_m$ - monotone submodular functions, $k$ -- a cardinality constraint
\begin{algorithmic}[1]
\State $S_1\gets \emptyset$\\
\For each element $e\in N$
\If{there exists $i\in[m]$ such that $f_i(e|S_1)\ge e^3(V_i - f_i(S_1))$ and $f_i(S_1) < (1-1/e)V_i$} $S_1\gets S_1\cap \{e\}$
\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

We may assume that for the output $S_1$ it holds $f_i(S_1)<(1-1/e)V_i$ for every $i\in[m]$ (as the submodular constraint would be already satisfied for the respective index $i$ otherwise).
\begin{lemma}\cite[~Lemma 5]{udwani2021multiobjective}
    Routine \ref{pr} outputs a set $S_1$ of size at most $m/\veps^3$. For each $e\in N-S_1$ it holds $f_i(S_1)\le \veps^3(V_i - f_i(S_1))$
\end{lemma}
where the notation $f(S'|S)$ means $f(S'\cap S) - f(S)$.

\textbf{Stage 2.} Now we are solving an LP on the ground set $N-S_1$ with the objective functions $F_i(\cdot | 1_{S_1})$ with $F_i$ being a multilinear extension of $f_i$ defined on $N$. This stage would use the continuous greedy algorithm \cite{10.1007/978-3-540-72792-7_15} to find a fractional solution ...

\textbf{Stage 3.} This is the final stage where we need to round the fractional solution obtained at stage 2 to a define a valid set $S$ that satisfies (...) whp. Udwani uses independent rounding adding element $i$ to $S_2$ with probability $(1 - \sqrt{\frac{\ln k_1}{k_1}})x_i$, where $k_1 = |N-S_1|$. Then by Chernoff inequality $|S_2|\le k_1$ with probability at most $e^{-\frac{\ln k_1}{3}}$. We take a different approach and use the dependent rounding scheme of \cite{Srinivasan2001DistributionsOL}:\\
In order to round the fractional solution vector $x = (x_1,\cdots, x_n\in [0,1]^n$ to a vector $X = (X_1, \cdots, X_n)\in \{0,1\}^n$ we deal with only two fractional values at a time. At time $0$ start with $X = x$. At each time-step with pick two indices $1\le i ,j\le n$ s.t. $X_i, X_j\ne\in \{0,1\}$, i.e., the values of $X_i$ and $X_j$ are still fractional. We update the values of $X_i$ and $X_j$ according to a case it falls into:\\
\texttt{\underline{Case I.}}
$0 < X_i+X_j <1$. Update 
$$
(X_i, X_j) = 
\begin{cases}
    (X_i+X_j, 0)\text{ with probability } \frac{X_i}{X_i+X_j};\\
    (0, X_i+X_j)\text{ with probability } \frac{X_j}{X_i+X_j}.
\end{cases}
$$
\texttt{\underline{Case II.}}
$X_i+X_j =1$. Update 
$$
(X_i, X_j) = 
\begin{cases}
    (1, 0)\text{ with probability } X_i;\\
    (0,1 )\text{ with probability } X_j.
\end{cases}
$$\texttt{\underline{Case III.}}
$1 < X_i+X_j < 2$. Update 
$$
(X_i, X_j) = 
\begin{cases}
    (X_i+X_j-1, 1)\text{ with probability } \frac{1-X_i}{1-(X_i+X_j)};\\
    (1, X_i+X_j-1)\text{ with probability } \frac{1-X_j}{1-(X_i+X_j)}.
\end{cases}
$$
The procedure is valid\cite{Srinivasan2001DistributionsOL}. If after $n-1$ steps there is still some value $X_i$ that is fractional (note that this can only happen if $\sum_ix_i<k_1$), then we round it to $1$ with probability $X_i$, and to $0$ otherwise. \rv{note sure if updating x instead of X would be better, but those are random variables, so...}. In the following we treat $X$ after the rounding occurred. 
\begin{theorem}
    \begin{enumerate}
        \item $\Pr[X_i = 1] = x_i$;\\
        \item The distribution of $X$ by applying Srinivasan's sampling process to the variables in any pre-determined order satisfies NA. \cite{DBLP:journals/cpc/DubhashiJR07}
    \end{enumerate}
\end{theorem}
Hence, we can apply theorem \ref{thm:main-concentration} to the algorithm.

\subsection{Analysis}
Let us prove \ref{thm: multi-obj}. The main fact from \cite{udwani2021multiobjective} that we state without proving it is that after finding the initial set $S_1$ is stage 1 and obtaining the fractional solution $x$ in stage 2 with $|x| = k_1 = k - |S_1|$ we have
that $$F_i(x|x_{S_1})\ge (1-1/e)\frac{k_1}{k}(V_i - f_i(S_1))\text{ for every }i.$$
Applying \ref{thm:main-concentration} we claim that the following bound holds whp:
\begin{align}\label{multi:ineq}
f_i(S_2|S_1) \ge (1-\veps)(1-1/e)\frac{k_1}{k}(V_i - f_i(S_1))\text{ for every }i.    
\end{align}
The probability it doesn't hold for some $i$ is
$$
\Pr[f_i(S_2|S_1) < (1-\veps)(1-1/e)\frac{k_1}{k}(V_i - f_i(S_1))]<
\Pr[f_i(S_2|S_1) < (1-\veps)F(x|x_{S_1})]
$$
Remember that [...scaling], hence, by \ref{thm:main-concentration}
$$
\Pr[f_i(S_2|S_1) < (1-\veps)F(x|x_{S_1})]
< e^{-\frac{F(x|x_{S_1})}{2\eps
(V_i - 
f_i
(S_1)
)}} 
< e^{-\frac{1-1/e}{2\veps}}.
$$
Therefore, by the union bound \ref{multi:ineq} holds when $\veps = O(\log m)$. And the factor in \ref{multi:ineq} tends to $(1-1/e)$ as $k\to\infty$ under the assumption $m = o(\frac{k}{\log ^3 k})$.
